On Causal Inference with Model-Based Outcomes

We study the estimation of causal effects on group-level parameters identified from microdata (e.g., child penalties). We demonstrate that standard one-step methods (such as pooled OLS and IV regressions) are generally inconsistent due to an endogenous weighting bias, where the policy affects the implicit weights (e.g., altering fertility rates). In contrast, we advocate for a two-step Minimum Distance (MD) framework that explicitly separates parameter identification from policy evaluation. This approach eliminates the endogenous weighting bias and requires explicitly confronting sample selection when groups are small, thereby improving transparency. We show that the MD estimator performs well when parameters can be estimated for most groups, and propose a robust alternative that uses auxiliary information in settings with limited data. To illustrate the importance of this methodological choice, we evaluate the effect of the 2005 Dutch childcare reform on child penalties and find that the conventional one-step approach yields estimates that are substantially larger than those from the two-step method.

==> sections/figAndTable.tex <==
 


\begin{comment}
 \begin{figure}[ht]
    \centering
    \caption{Effect of childcare expansion: continuous MD approach}
    \label{fig:did_1vs4}
        \centering
        \includegraphics[width=0.95\textwidth]{\outputDir/onestep2x2.pdf}
    
    \caption*{
        \footnotesize \textit{Notes:}
        This figure presents discrete difference-in-differences estimates of the effects of the childcare expansion on child penalties, described in Section \ref{sec:compareCommonMethods}. The pre-/post-period are 2000-2005 and 2011-2016, and the treatment group is defined as the municipality where the childcare index increased by 10 percentages points from the pre-period to the post-period. Our childcare supply index ($CCI$) for each municipality is calculated by dividing the number of childcare jobs in a given municipality $m$ and year $t$ ($N^{jobs}_{g,t}$) by the number of children under 5 years of age in the same locality ($ N_{g,t}^{children})$
    }
    
\end{figure}

\end{comment}


==> sections/garbage.tex <==
@misc{Decree1996,
  title        = {Childcare Quality Requirements (Temporary Measures) Decree, 1996},
  year         = {1996},
  note         = {Available via SPLASH Policy Document Database},
  howpublished = {\url{https://splash-db.eu/?cHash=3d3f1e98078d34205fd2c1a80af9ff46&tx_perfar_policydocument[action]=show&tx_perfar_policydocument[controller]=Policydocument&tx_perfar_policydocument[policydocument]=1352}}
}




%\footnote{Note that we adjusted our sample criteria to include parents with their first childbirth after 1995 to allow for a sufficient labor market horizon (e.g., to observe the horizon $h=5$ at 2000). Furthermore, since the one-step approach does not typically segment the analysis by education, we remove the age at first birth criteria by education group, instead including all parents whose age at first birth is between 24 and 34, regardless of their education level (high school, vocational, or bachelors).}

    \tz{This is our old measure, below I suggest the adjusted one, if we want to explore it in the updated exercise.}
    
    To create a municipality-based index of childcare supply, we use comprehensive information from the 5-digit sector classification, which has been available for all jobs in the Netherlands since 2001. These data allow us to identify childcare workers and their job locations.\footnote{\cite{Rabate2021} Appendix C.2 shows a strong correlation between the trends in childcare employment and the aggregate public spending on childcare, validating this index.} Our childcare supply index ($CCI$) for each municipality is calculated by dividing the number of childcare jobs in a given municipality $g$ and year $t$ ($N^{jobs}_{g,t}$)  by the number of children under 5 years of age in the same locality ($N_{g,t}^{children}$):
    %
    \begin{equation*}
        CCI_{g,t} = N^{jobs}_{g,t}/ N_{g,t}^{children} 
    \end{equation*}
    %
    
    
    \tz{Dmitry do we still want to explore the adjusted CCI in the updated exercise:}
    
    Childcare Supply Index Definition:
    Based on the official child-to-staff ratios established by the Netherlands’ Childcare Quality Requirements (Temporary Measures) Decree of 1996 \cite{Decree1996}, we define a municipality-level Childcare Capacity Index ($CCI_{g,t}$) that captures the ratio of the available childcare workforce to the effective demand for childcare, where demand is scaled by the legally required staffing per child at each age. Formally, for municipality $g$ in year $t$:
    %
    \begin{align*}
        CCI_{g, t} = \frac{J_{g, t}}{\sum_{h=0}^{5} \frac{N_{g, t, h}}{R_h}}
    \end{align*}
    %
    where $J_{g,t}$ is the number of childcare workers in municipality $g$ at time $t$, $N_{g,t,h}$ is the number of children of age $h \in {0,\dots,5}$, and $R_h$ is the legal child-to-staff ratio for that age group. The statutory values are $R_0=4$, $R_1=5$, $R_2=6$, $R_3=8$, and $R_4 = R_5 = 10$ as stipulated by the 1996 decree \cite{Decree1996}.
    
    This index thus measures the relative sufficiency of childcare supply—interpretable as the number of children that could be served per job, adjusted for age-specific staff requirements. A value of 1 implies that the number of childcare jobs exactly meets the regulated staffing requirement for the existing population of 0–5-year-olds in that municipality-year.

    \tz{End of new measure}
    
    Figure \ref{fig:cci_dist} presents the variation in childcare supply per preschool-aged child across municipalities from 1999 to 2016. Each dot represents the mean $CCI$ in a given year, whereas the shaded area represents the distribution of $CCI$ across municipalities. The data reveal a significant range in the ratio of childcare workers to preschool children, with values ranging from 0 to 0.3.\footnote{Measurement errors might influence some of the extreme values since the job location is tied to the firm's location and may not always align with the actual municipality where the job is performed.} The figure illustrates the substantial variation in childcare availability between different municipalities and the large increase due to the 2005 childcare expansion reform.
    

    
    \begin{remark}\label{rem:supplyVSdemandCCI}
    \textbf{Interpreting childcare capacity as a moderating treatment.}
    Our empirical design examines how the child penalty varies with local childcare provision, effectively treating the interaction between childbirth and childcare capacity as a two-dimensional treatment. While the Childcare Capacity Index ($CCI_{g,t}$) reflects an equilibrium outcome shaped by local supply and demand, we view it as an exogenous shock from the individual’s perspective—capturing variation in the childcare environment at the time of childbirth.
    

    \end{remark}
\da{Potentially relevant references: \cite{paravisini2015dissecting} (literally doing what we do but with IV and without local markets, simply relating $\psi_b$ to something about $b$), \cite{jimenez2012credit} (seem to be doing something similar, but over time rather than space), \cite{jimenez2017macroprudential} (also seem to be relevant). Potentially \cite{bolton2016relationship} (over time, not space).}



\subsection{Derivations for IV}

The parameter of interest in this example is $\beta$. A common empirical practice is to estimate it using TSLS for the following equation:
%
\begin{equation*} 
Y_{g,i} = \delta_g + (\alpha+ \beta W_g) X_{g,i} + \varepsilon_{g,i}.
\end{equation*}
%
Here the two endogenous regressors $X_{g,i}$ and $W_gX_{g,i}$ are instrumented using $\tilde X_{g,i}$ and $Z_g\tilde X_{g,i}$. Consider a population limit where $G \rightarrow \infty$ and $n\rightarrow \infty$. 


Let $\bm{\beta}^{RF}$ be a vector of population reduced form coefficients in the regression of $Y_{g,i}$ on $Z_{g,i}:= (Z_g - \mu_z)(\tilde{X}_{g,i} - \mathbb{E}_{F_g}[\tilde{X}_{g,i}])$ and $\tilde{X}_{g,i}^{\star} := (\tilde{X}_{g,i} - \mathbb{E}_{F_g}[\tilde{X}_{g,i}])$
Also let $\Pi$ be a $2\times 2$ matrix of population first stage coefficients in regressing $X_{g,i}W_{g}$ and $X_{g,i}$ on the same things (each column of $\Pi$ corresponds to the corresponding coefficients). Then we have that $\beta^{TSLS}$ (the population limit is equal to) the first component of the vector $\Pi^{-1}\bm{\beta}^{RF}$, or computing the inverse, it is equal to
%
\begin{equation*}
    \beta^{TSLS} = \frac{\beta_1^{RF} - \frac{\Pi_{1,2}}{\Pi_{2,2}} \beta_2^{RF}}{\Pi_{1,1} - \frac{\Pi_{1,2}}{\Pi_{2,2}}\Pi_{2,1} }
\end{equation*}
%
Let $C_g :=\E_{F_g}[X_{g,i}(\tilde{X}_{g,i} - \mathbb{E}_{F_g}[\tilde{X}_{g,i}])]$  be the group-specific covariance between $X_{g,i}$ and $\tilde X_{g,i}$. We now compute each component of the formula for $\beta^{TSLS}$
We have
\begin{align*}
    &\beta_1^{RF} = \frac{\E[\E_{F_g}[Y_{g,i} Z_{g,i}]]}{\Var[Z_{g,i}]} = \frac{\E[C_g\alpha_g(Z_g - \mu_z) + \beta C_gW_g(Z_g - \mu_z)]}{\Var[Z_{g,i}]}\\
    &\beta_2^{RF} =\frac{\E[\E_{F_g}[Y_{g,i} \tilde{X}_{g,i}^{\star}]]}{\Var[ \tilde{X}_{g,i}^{\star}]} = \frac{\E[C_g(\alpha_g + \beta W_g) ]}{ \Var[\tilde{X}_{g,i}^{\star}]}\\
    &\Pi_{1,1} = \frac{\E[\E_{F_g}[X_{g,i}W_{g} Z_{g,i}]]}{\Var[Z_{g,i}]} = \frac{\E[C_gW_g(Z_g - \mu_z)]}{\Var[Z_{g,i}]}\\
    &\Pi_{2,2} = \frac{\E[\E_{F_g}[X_{g,i} \tilde X^{\star}_{g,i}]]}{\Var[\tilde X^{\star}_{g,i}]} = \frac{\E[C_g]}{\Var[\tilde X^{\star}_{g,i}]}\\
    &\Pi_{1,2} =  \frac{\E[\E_{F_g}[X_{g,i} Z_{g,i}]]}{\Var[Z_{g,i}]} = \frac{\E[C_g(Z_g - \mu_z) ]}{ \Var[Z_{g,i}]}\\
    &\Pi_{2,1} = \frac{\E[\E_{F_g}[X_{g,i}W_{g} \tilde X^{\star}_{g,i}]]}{\Var[\tilde X^{\star}_{g,i}]} =  \frac{\E[C_gW_{g} ]}{\Var[\tilde X^{\star}_{g,i}]}
\end{align*}


Substituting these expressions we get the following for the numerator:
\begin{align*}
    \frac{1}{\Var[Z_{g,i}]}\left(\E[C_g\alpha_g(Z_g - \mu_z) + \beta C_gW_g(Z_g - \mu_z)] -\frac{\E[C_g(Z_g - \mu_z) ]}{\E[C_g]} \E[C_g(\alpha_g + \beta W_g) ]\right)
\end{align*}
For the denominator we get
\begin{align*}
    \frac{1}{\Var[Z_{g,i}]}\left(\E[C_gW_g(Z_g - \mu_z)] -\frac{\E[C_g(Z_g - \mu_z) ]}{\E[C_g]} \E[C_gW_{g} ]\right)
\end{align*}
Rearranging the terms and simplifying we get the following expression:
\begin{align*}
    \beta^{TSLS} = \frac{\E[C_g\alpha_g(Z_g - \tilde \mu_z) + \beta C_gW_g(Z_g - \tilde\mu_z)]}{\E[C_gW_g(Z_g - \tilde\mu_z)]} = \frac{\Cov_{C_g}[\tau_g,Z_g]}{\Cov_{C_g}[W_g,Z_g]} = \\
    \beta + \frac{\Cov_{C_g}[\alpha_g,Z_g]}{\Cov_{C_g}[W_g,Z_g]}
\end{align*}
where $\tilde \mu_z :=\frac{\E[C_g Z_g ]}{\E[C_g]}$ the mean with respect to the measure (potentially negative valued) of $Z_g$, and $\Cov_{C_g}$ is the covariance using the same measure. 

\appendix
\section{Derivation of GMM Weights and Bias for the Banking Example}\label{app:banking_weight_derivation}

This appendix details the derivation of the policy-dependent GMM weights and the resulting bias formula for the banking deregulation example, as discussed in Section~\ref{sec:gmm_bias_banking_derived}, based on the setup in Section~\ref{sec:example_banking_deregulation_revised}.

We assume that in each market $g$, for the identification of $\bm{\theta}_g = (\psi_{g,2}, \psi_{g,3})^\top$ (with $\psi_{g,1} \equiv 0$), we observe firms that interact either with banks of types 1 and 2 (Type A firms, $K_A$) or types 1 and 3 (Type B firms, $K_B$). No firms used for this identification interact only with types 2 and 3, or with all three types.

The parameters $\bm{\theta}_g$ are identified from the moment conditions:
%
\begin{equation}\label{eq:app_banking_moments_theta}
    \mathbb{E}_{F_g}\left[X_{g,i}(\Delta Y_{g,i}^* - X_{g,i}^\top \bm{\theta}_g)\right] = \mathbf{0}_2,
\end{equation}
%
where $X_{g,i} = (\mathbf{1}\{K_{g,i}=K_A\}, \mathbf{1}\{K_{g,i}=K_B\})^\top$, and the scalar outcome $\Delta Y_{g,i}^*$ is defined as:
%
\begin{equation*}
    \Delta Y_{g,i}^* = \mathbf{1}\{K_{g,i}=K_A\}(Y_{g,i,2} - Y_{g,i,1}) + \mathbf{1}\{K_{g,i}=K_B\}(Y_{g,i,3} - Y_{g,i,1}).
\end{equation*}
%
The matrix of second moments of the regressors $X_{g,i}$ is:
%
\begin{equation}\label{eq:app_banking_Atilde}
    \tilde A_g = \mathbb{E}_{F_g}[X_{g,i} X_{g,i}^\top] = \begin{pmatrix} \mathbb{P}_{F_g}(K_A) & 0 \\ 0 & \mathbb{P}_{F_g}(K_B) \end{pmatrix} = \operatorname{diag}\{p_{gA}, p_{gB}\},
\end{equation}
%
where $p_{gA} = \mathbb{P}_{F_g}(K_A)$ and $p_{gB} = \mathbb{P}_{F_g}(K_B)$. If policy $W_g$ affects $p_{gA}$ or $p_{gB}$, then $\tilde A_g = \tilde A_g(W_g)$.

We assume the structural model for bank-type specific effects is:
%
\begin{equation*}
    \psi_{g,b} = u_{g,b} + \beta_0 W_{g,b} \quad \text{for } b \in \{2,3\},
\end{equation*}
%
where $u_{g,b}$ is unobserved heterogeneity (e.g., incorporating baseline bank-type effects $\alpha_b$, common group effects $\lambda_g$, and further group-bank specific heterogeneity $\alpha_{g,b}$ from other conceptualizations), and $W_{g,b}$ is the policy measure relevant for bank type $b$. The parameter $\beta_0$ captures the policy's effect.

The one-step GMM estimator for $\beta_0$ can be conceptualized through a population weighted least squares problem. If we consider estimating $(\alpha_b, \beta_0)$ and common group effects $\lambda_g$ from the system for $b=2,3$:
%
\begin{equation*}
  \min_{\{\alpha_b\}, \beta_0} \mathbb{E}_g \left[ \min_{\lambda_g} \sum_{b=2,3} p_{gb}(W_g) (\psi_{g,b} - \lambda_g - \alpha_b - \beta_0 W_{g,b})^2 \right],
\end{equation*}
%
where $p_{g2}(W_g) = p_{gA}(W_g)$ and $p_{g3}(W_g) = p_{gB}(W_g)$ are the policy-dependent probabilities from $\tilde A_g(W_g)$, acting as weights.
The inner minimization yields:
%
\begin{equation*}
    \hat{\lambda}_g = \frac{\sum_{b=2,3} p_{gb}(W_g)(\psi_{g,b} - \alpha_b - \beta_0 W_{g,b})}{\sum_{b=2,3} p_{gb}(W_g)}.
\end{equation*}
%
Substituting $\hat{\lambda}_g$ back into the objective function, the problem reduces to minimizing (over $\Delta\alpha = \alpha_3-\alpha_2$ and $\beta_0$):
%
\begin{equation*}
    \min_{\Delta\alpha, \beta_0} \mathbb{E}_g \left[ w_g(W_g) (\Delta\psi_g - \Delta\alpha - \beta_0 \Delta W_g)^2 \right],
\end{equation*}
%
where $\Delta\psi_g = \psi_{g,3} - \psi_{g,2}$, $\Delta W_g = W_{g,3} - W_{g,2}$ (the effective policy regressor for the difference), and the effective weight is:
%
\begin{equation}\label{eq:app_banking_weight_wg}
    w_g(W_g) = \frac{p_{gA}(W_g) p_{gB}(W_g)}{(p_{gA}(W_g) + p_{gB}(W_g))^2}.
\end{equation}
%
The GMM estimator $\hat{\beta}^{GMM}$ for $\beta_0$ converges to:
%
\begin{equation*}
    \plim_{G\to\infty} \hat{\beta}^{GMM} = \frac{\operatorname{Cov}^{w_g(W_g)}[\Delta\psi_g, \Delta W_g]}{\operatorname{Var}^{w_g(W_g)}[\Delta W_g]}.
\end{equation*}
%
Substituting $\Delta\psi_g = \Delta u_g + \beta_0 \Delta W_g$ (where $\Delta u_g = u_{g,3}-u_{g,2}$ is the relevant unobserved heterogeneity), the asymptotic bias is:
%
\begin{equation}\label{eq:app_bias_banking_final}
    \plim_{G\to\infty} (\hat{\beta}^{GMM} - \beta_0) = \frac{\operatorname{Cov}^{w_g(W_g)}[\Delta u_g, \Delta W_g]}{\operatorname{Var}^{w_g(W_g)}[\Delta W_g]}.
\end{equation}
%
This bias arises if $w_g(W_g)$ (which depends on policy $W_g$ through $p_{gA}(W_g)$ and $p_{gB}(W_g)$) induces a correlation between $\Delta W_g$ and the heterogeneity $\Delta u_g$.
